Optimal Sequence-Based Control and Estimation of Networked Linear Systems

In this paper, a unified approach to sequence-based control and estimation of linear networked systems with multiple sensors is proposed. Time delays and data losses in the controller-actuator-channel are compensated by sending sequences of control inputs. The sequence-based design paradigm is further extended to the sensor-controller-channels without increasing the load of the network. In this context, we present a recursive solution based on the Hypothesizing Distributed Kalman Filter (HKF) that is included in the overall sequence-based controller design.

==> OutOfSequenceCI.tex <==
Basic formulas
\begin{align}
\infDelta{i}{k+1} = \infA{k} \infDelta{i}{k} \inv{\infA{k}} \\
\infDelta{i}{k|k} = \infK{k} \infDelta{i}{k} + \infL{i}{k} \infH{i}{k} \\
\infDelta{i}{k} = \infK{k} \infA{k-1} \infDelta{i}{k-1} \inv{\infA{k-1}} + \infL{i}{k} \infH{i}{k}
\end{align}

\begin{align}
\infx{i}{k+1} = \infA{k} \infx{i}{k} \\
\infx{i}{k|k} = \infK{k} \infx{i}{k} + \infL{i}{k} \truez{i}{k}
\end{align}

\textbf{Actually utilized gains for HKF processing}

\begin{align}
\infDelta{i}{k} = \sum_{t=1}^k \infG{t:k} \infL{i}{t} \infH{i}{t} \inv{\infA{t:k}}
\end{align}
with
\begin{align}
\infG{l:k} = \bigg( \prod_{t=l}^{k-1} \transpose{\infA{t}} \transpose{\infK{t+1}}  \bigg)^\top
\end{align}
and
\begin{align}
\inv{\infA{l:k}} = \prod_{t=l}^{k-1} \inv{\infA{t}}
\end{align}

\begin{align}
\infx{i}{k} = \sum_{t=1}^k \infG{t:k} \infL{i}{t} \truez{i}{t}
\end{align}



Single estimate is given by
\begin{align}
\inv{\infDelta{i}{k}} \infx{i}{k} =&  \sum_{t=1}^k \inv{\infDelta{i}{k}} \infG{t:k} \infL{i}{t} \truez{i}{t} \\
=& \sum_{t=1}^k \Big( \inv{\infG{t:k}} \infDelta{i}{k}  \Big)^{-1} \infL{i}{t} \truez{i}{t} \\
=& \sum_{t=1}^k \Big( \sum_{l=1}^k \inv{\infG{t:k}} \infG{l:k} \infL{i}{l} \infH{i}{l} \inv{\infA{l:k}}  \Big)^{-1} \infL{i}{t} \truez{i}{t}  \\
=& \sum_{t=1}^k \Big( \sum_{l=1}^k \infG{l:t} \infL{i}{l} \infH{i}{l} \inv{\infA{l:k}}  \Big)^{-1} \infL{i}{t} \truez{i}{t}
\end{align}
where
\begin{align}
\infG{l:t} = \inv{\infG{t:l}} \text{ when } l > t 
\end{align}

Fused estimate
\begin{align}
\infDelta{f}{k} = \sum_{i \in G_f} \infDelta{i}{k} \\
\infx{f}{k} = \sum_{i \in G_f} \infx{i}{k}
\end{align}

\begin{align}
\label{eq:estxfused}
\inv{\infDelta{f}{k}} \infx{f}{k}
=& \sum_{t=1}^k \Big( \inv{\infG{t:k}} \infDelta{f}{k}  \Big)^{-1} \Big( \sum_{i \in G_f} \infL{i}{t} \truez{i}{t} \Big) \\
=& \sum_{t=1}^k \Big( \inv{\infG{t:k}} \infDelta{f}{k}  \Big)^{-1} \Big( \sum_{i \in G_f} \infL{i}{t} \truez{i}{t} \Big)
\end{align}
with
\begin{align}
\infDelta{f}{k} = \sum_{t=1}^k \infG{t:k} \Big(  \sum_{i \in G_f} \infL{i}{t} \infH{i}{t} \Big) \inv{\infA{t:k}}
\end{align}

\paragraph{What part of u is already included in the estimate?}

In the following we take into account only the mean values. When we assume that the initial state can be represented by $\truex{0} = \infB{0} \trueu{0}$, we obtain for the mean values of the measurements
\begin{align}
\truez{i}{t} = \infH{i}{t} \sum_{l=0}^{t-1} \infA{l+1:t} \infB{l} \trueu{l} 
\end{align}
with
\begin{align}
 \infA{t:t} = \mat{I}
\end{align}
From~\eqref{eq:estxfused} we obtain for $\inv{\infDelta{f}{k}} \infx{f}{k}$
\begin{align}
\sum_{t=1}^k \inv{\infDelta{f}{k}} \infG{t:k} \Big( \sum_{i \in G_f} \infL{i}{t} \truez{i}{t} \Big) \\ = 
\sum_{t=1}^k \inv{\infDelta{f}{k}} \infG{t:k} \Big( \sum_{i \in G_f} \infL{i}{t} \infH{i}{t} \sum_{l=0}^{t-1} \infA{l+1:t} \infB{l} \trueu{l}  \Big)
\end{align}

We transform the term so that the inputs are separated
\begin{align}
\inv{\infDelta{f}{k}}  \sum_{t=1}^k \infG{t:k} \Big( \sum_{i \in G_f} \infL{i}{t} \infH{i}{t}  \Big)  \sum_{l=0}^{t-1} \infA{l+1:t} \infB{l} \trueu{l} \\
= \inv{\infDelta{f}{k}}  \sum_{t=0}^{k-1}  \bigg( \sum_{l=t+1}^k \infG{l:k} \Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) \infA{t+1:l} \bigg) \infB{t} \trueu{t}
\end{align}

Each input must be included according to its part of the state at time step $k$. As this part is given by $\infA{t+1:k} \infB{t} \trueu{t}$, it must hold
\begin{align}
\inv{\infDelta{f}{k}} \sum_{l=t+1}^k \infG{l:k} \Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) \infA{t+1:l} + \mat{G}^u_{t+1:k} = \infA{t+1:k}
\end{align}
and thus $\mat{G}^u_{t+1:k}$ is given by
\begin{align}
\bigg( \mat{I} - \inv{\infDelta{f}{k}} \sum_{l=t+1}^k \infG{l:k} \Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) \inv{\infA{l:k}} \bigg) \infA{t+1:k}  \\
= \inv{\infDelta{f}{k}} \bigg( \sum_{l=1}^k \infG{l:k}  \Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) \inv{\infA{l:k}} - \\ \sum_{l=t+1}^k \infG{l:k} \Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) \inv{\infA{l:k}} \bigg) \infA{t+1:k} \\
= \inv{\infDelta{f}{k}} \bigg( \sum_{l=1}^t \infG{l:k}  \Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) \inv{\infA{l:k}} \bigg) \infA{t+1:k} \\
= \inv{\infDelta{f}{k}} \infG{t+1:k} \bigg( \sum_{l=1}^t \infG{l:t}  \Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) \inv{\infA{l:t}} \bigg) \\
%= \inv{\infDelta{f}{k}} \infG{t+1:k} \infDelta{f}{t} \inv{\infA{t+1:k}}  \infA{t+1:k} \\
= \inv{\infDelta{f}{k}} \infG{t+1:k} \infDelta{f}{t} \text{ .}
\end{align}

%\begin{align}
%\infDelta{f}{k} \mat{G}^u_{t+1:k} = \infG{t:k} \inv{\infG{t}} \bigg( 
%\infK{t} \infA{t-1} \infDelta{f}{t-1} \inv{\infA{t-1}} + \\
%\Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) \bigg) \\
%= \infG{t:k} \infDelta{f}{t-1} \inv{\infA{t-1}} + \inv{\infG{t}} \Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) \\
%= \infDelta{f}{k} \mat{G}^u_{t:k} \inv{\infA{t-1}} + \inv{\infG{t}} \Big( \sum_{i \in G_f} \infL{i}{l} \infH{i}{l} \Big) 
%\end{align}

It remains to calculate
\begin{align}
\inv{\infDelta{f}{k}} \sum_{t=1}^k \infG{t+1:k} \infDelta{f}{t} \infB{t} \trueu{t} \text{. }
\end{align}
When we assume that the control input is constant over the time sequence $1,\dots,k$, this equation is simplified to 
\begin{align}
\inv{\infDelta{f}{k}} \sum_{t=1}^k \infG{t+1:k} \infDelta{f}{t} \vec{b} 
\end{align}
with $\vec{b} = const$. Thus, we can transform the formula to
\begin{align}
\sum_{t=1}^k \infG{t+1:k} \infDelta{f}{t} =&
\sum_{t=1}^k \infG{t+1:k} \sum_{i\in G_f} \infDelta{i}{t} \\
=& \sum_{i \in G_f} \sum_{t=1}^k \infG{t+1:k} \infDelta{i}{t} \text{ .} 
\end{align}
However, as we can calculate the inner sum $\sum_{t=1}^k \infG{t+1:k} \infDelta{i}{t}$ locally at each node, only one $\mathbb{R}^{n x n}$ matrix must be transmitted to the fusion center in order to allow the control input correction later on.


%::::CRAP:::: 
%
%Constant models (A, K, fixed)
%\begin{align}
%\infA{l:k} = \big( \infA{} \big)^{k-l+1} \\
%\infG{l:k} = \big( \infK{} \infA{} \big)^{k-l+1}
%\end{align}
%and thus
%\begin{align}
%\inv{\infDelta{f}{k}} \infx{f}{k} = 
%\sum_{t=1}^k \Big( \sum_{l=1}^k \big( \infK{} \infA{} \big)^{t-l} \sum_{i \in G_f} \Big( \infL{i}{t} \infH{i}{t} \Big) \big( \infA{} \big)^{l-k-1} \Big)^{-1} \infL{i}{t} \truez{i}{t} 
%\end{align}
